ScaleDisturb: Exploiting Temporal Asymmetry to Amplify Read Disturbance in Modern DRAM Chips

DRAM suffers from read disturbance phenomena (e.g., RowHammer and RowPress), where repeatedly accessing or continuously keeping open a DRAM row (aggressor row) induces bitflips in other physically nearby unaccessed rows (victim rows). The disturbance mechanism is practically exploitable from the software stack and worsens across generations with continued density scaling. DRAM read disturbance is highly sensitive to memory access patterns, yet prior work explores read disturbance under only a limited set of access patterns. We present ScaleDisturb, a new DRAM access pattern that can amplify DRAM read disturbance by asymmetrically extending the open time of two aggressor rows. Our rigorous experimental characterization of 196 DDR4 and 3 HBM2 DRAM chips shows that ScaleDisturb (1) leads to bitflips at significantly fewer row activations, compared to state-of-the-art memory access patterns, (2) makes read disturbance attacks easier across all tested DRAM chips, (3) increases DRAM vulnerability to read disturbance as DRAM manufacturing technology scales down to smaller node sizes. We showcase a proof-of-concept attack on a real system where a user-level program leveraging ScaleDisturb induces more bitflips than state-of-the-art RowHammer and RowPress memory access patterns. We describe and evaluate four solutions for mitigating read disturbance bitflips in the presence of ScaleDisturb and call for more research on the topic.

==> hpca-template.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% -- DO NOT MODIFY -- %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\author{
  \ifdefined\hpcacameraready
    \IEEEauthorblockN{\hpcaauthors{}}
      \IEEEauthorblockA{
        \hpcaaffiliation{} \\
        \hpcaemail{}
      }
  \else
    \IEEEauthorblockN{\normalsize{HPCA \hpcayear{} Submission
      \textbf{\#\hpcasubmissionnumber{}}} \\
      \IEEEauthorblockA{
        Confidential Draft \\
        Do NOT Distribute!!
      }
    }
  \fi 
}

% Heading and footer for title page
\fancypagestyle{camerareadyfirstpage}{%
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[C]{
    \ifdefined\aeopen
    \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}    
    \else
      \ifdefined\aereviewed
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \ifdefined\aereproduced
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \parbox[][0mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
    \fi 
    \fi 
    \fi 
    \ifdefined\aeopen 
      \includegraphics[width=12mm,height=12mm]{ae-badges/open-research-objects.pdf}
    \fi 
    \ifdefined\aereviewed
      \includegraphics[width=12mm,height=12mm]{ae-badges/research-objects-reviewed.pdf}
    \fi 
    \ifdefined\aereproduced
      \includegraphics[width=12mm,height=12mm]{ae-badges/results-reproduced.pdf}
    \fi
  }
  %\fancyfoot[L]{\hpcapubid{} \copyright \hpcayear{} IEEE}
  \fancyfoot[C]{}
}
% Heading and footer for remaining pages
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}
%\fancyhead[C]{\hpcayear{} IEEE International Symposium on
% High-Performance Computer Architecture (HPCA)}


\begin{document}
\maketitle

%Enables the camera ready header and footer
\ifdefined\hpcacameraready 
  \thispagestyle{camerareadyfirstpage}
  \pagestyle{empty}
\else
  \thispagestyle{plain}
  \pagestyle{plain}
\fi

\newcommand{\hpcaheight}{0mm}
\ifdefined\eaopen
\renewcommand{\hpcaheight}{12mm}
\fi
  


==> sections/3motivation.tex <==
\section{Motivation}
The read disturbance has significant implications for the robustness of the system (i.e., reliability, security, and safety), as it is widespread and can be exploited to break memory isolation~\cite{kim2014flipping,frigo2020trrespass, orosa2021deeper, hassan2021utrr, kogler2022half, luo2023rowpress, luo2024experimental, luo2025revisiting,tol2023dontknock,liu2023hyperattack,dong2023onebitfilp,staudigl2022neurohammer,roohi2022efficient,cai2022feasibility}. The robustness guarantees provided by existing read disturbance mitigations rely on accurately characterizing the minimal activation count, typically evaluated under existing memory access patterns~\cite{seyedzadeh2018cbt,yaglikci2021blockhammer,park2020graphene,qureshi2022hydra,saileshwar2022randomized,kim2022mithril,marazzi2023rega,saxena2022aqua,saroiu2022configure,olgun2024abacus,yaglikci2024svard,bostanci2024comet,saxena2024start,saxena2024rubix}. Unfortunately, previous studies cumulatively examine \emph{only} a narrow subset of all possible memory access scenarios. Our \textbf{goal} in this paper is to explore \rbi{a} DRAM access \rbi{pattern} that can reduce the minimum aggressor row activation count to induce bitflips compared to access patterns characterized in prior works, and 2) understand its implications for the secure, reliable, and safe operation of DRAM-based systems.


==> sections/abstractclean.tex <==
\begin{abstract}

DRAM suffers from read disturbance phenomena (e.g., RowHammer and RowPress), where repeatedly accessing or continuously keeping open a DRAM row (aggressor row) induces bitflips in other physically nearby \emph{unaccessed} rows (victim rows). The disturbance mechanism is practically exploitable from the software stack and worsens across generations with continued density scaling. DRAM read disturbance is highly sensitive to memory access patterns, yet prior work explores read disturbance under only a \emph{limited} set of access patterns.

In this work, we present ScaleDisturb, a new DRAM access pattern that can amplify DRAM read disturbance by asymmetrically extending the open time of two aggressor rows. Our rigorous experimental characterization of 196 DDR4 and 3 HBM2 DRAM chips shows that ScaleDisturb 
(1) leads to bitflips at significantly fewer row activations, compared to state-of-the-art memory access patterns,
(2) makes read disturbance attacks easier across all tested DRAM chips,
(3) increases DRAM vulnerability to read disturbance as DRAM manufacturing technology scales down.
We showcase a proof-of-concept attack on a real system where a user-level program leveraging ScaleDisturb induces more bitflips than state-of-the-art RowHammer and RowPress memory access patterns.
We describe and evaluate four solutions for mitigating read disturbance bitflips in the presence of ScaleDisturb and call for more research on the topic.

\end{abstract}
